RELIEF: Turning Missing Modalities into Training Acceleration for Federated Learning on Heterogeneous IoT Edge

Federated learning (FL) over heterogeneous IoT edge devices faces coupled system-modality-data heterogeneity: the lower-cost device carries both fewer sensors and less computational power, so the slowest device (straggler) produces the most incomplete gradient signals. Naively averaging their updates dilutes rare-modality information and wastes computation on absent-sensor parameters, whereas existing methods handle the triple heterogeneity (system, modality, data) in isolation and none addresses their coupling. To resolve this issue, we propose RELIEF, a framework that partitions the fusion-layer Low-Rank Adaptation (LoRA) projection matrix into modality-aligned column blocks and uses this partition as a unified interface for aggregation, elastic training, and communication. Each block is aggregated only within the cohort of devices possessing that modality, which eliminates cross-modal gradient interference; the server then allocates personalized training budgets by prioritizing blocks with the highest cohort-internal divergence, so that resource-constrained devices train fewer but more impactful parameters. We prove that cohort-wise aggregation removes interference from the convergence bound and that the divergence-guided allocation achieves sublinear regret. Experiments on two IoT sensor datasets (PAMAP2, MHEALTH) under both full-parameter (CNN) and parameter-efficient (LoRA) training show that RELIEF achieves up to 9.41x speedup and 37% energy reduction over FedAvg with up to 15.3 pp rare-modality F1 gains, and real-device validation on a two-Jetson AGX Orin testbed confirms these results.

==> section/5_experiment.tex <==
\section{Performance Evaluation}
\label{sec:experiments}

\subsection{Experimental Setup}

\subsubsection{Datasets}
We evaluate \method{} on two publicly available multimodal human activity recognition (HAR) datasets that reflect realistic IoT sensor heterogeneity.

\textbf{PAMAP2}~\cite{Reiss2012ISWC} contains data from 9 subjects wearing IMU sensors, covering 12 activity classes. Each subject provides four sensor modalities: accelerometer (Acc), gyroscope (Gyro), magnetometer (Mag), and heart rate (HR). Following prior work~\cite{Reiss2012ISWC}, we exclude Subject~9 due to insufficient recording length and partition the remaining 8 subjects into 8 FL clients, configured as 3$\times$Full (4 modalities, 1$\times$ compute), 3$\times$Acc+Gyro (2 modalities, 13$\times$ slower), and 2$\times$Acc-only (1 modality, 55$\times$ slower), reflecting the coupled cost gradient described in Section~\ref{sec:problem_formulation}.

\textbf{MHEALTH}~\cite{Banos2014IWAAL} records data from 10 subjects with four modalities: Acc, Gyro, Mag, and electrocardiogram (ECG), across 12 activity classes. We partition by subject into 10 clients: 3$\times$Full (1$\times$), 3$\times$Acc+Gyro (13$\times$), and 4$\times$Acc-only (55$\times$).

Both datasets use a sliding window of 5.12\,s (256 samples at 50\,Hz) with a 1\,s stride. We report macro-F1 as the primary metric, wall-clock speedup relative to FedAvg, and per-round communication volume.

\subsubsection{Baselines}
We compare against 10 methods spanning three categories.

\textit{Classical FL:}
FedAvg~\cite{McMahan2017AISTATS} and
FedProx~\cite{Li2020MLSys}.

\textit{System-heterogeneous / elastic FL:}
FedEL~\cite{Zhang2025NeurIPS},
FedICU~\cite{Liao2025ICML}, and
DarkDistill~\cite{Qu2025KDD}.

\textit{Multimodal FL / federated LoRA:}
Harmony~\cite{Ouyang2023MobiSys},
Pilot~\cite{Xiong2025AAAI},
FedSA-LoRA~\cite{Guo2025ICLR},
HeLoRA~\cite{Fan2025TOIT}, and
FedLEASE~\cite{Wang2025NeurIPS}.

All methods share identical data splits, device heterogeneity configurations, and communication protocols.

\subsubsection{Implementation Details}
We employ two backbone architectures to validate \method{} under both full-parameter and parameter-efficient training.

\textbf{Backbone~1 (lightweight CNN):} Each modality encoder is a 2-layer 1D-CNN with $<$2M total parameters. The fusion layer is a fully connected layer whose weight matrix is partitioned into modality-aligned column blocks for modality-decomposed aggregation.

\textbf{Backbone~2 (pretrained Transformer + LoRA):} Each modality encoder is an independent MOMENT~\cite{Goswami2024ICML} instance ($\sim$40M parameters, $\sim$160M total). We freeze the backbone and inject LoRA adapters ($\rho = 8$) into each attention layer's Q/V projections and the FFN, yielding $\sim$300K trainable parameters ($<$0.2\%). The fusion-layer LoRA projection matrix $A$ is partitioned into modality-aligned column blocks for MDLoRA.

Training uses Adam with learning rate $1\times10^{-3}$, batch size 32, $E = 5$ local epochs, and $R = 200$ rounds. The EMA coefficient is $\gamma = 0.9$. Device heterogeneity is simulated via FLOP-proportional profiling calibrated to edge TOPS: Full devices at 275 TOPS (Jetson AGX Orin level), Acc+Gyro at 21 TOPS (Xavier NX level), and Acc-only at 5 TOPS (low-end IoT level).

We estimate per-round fleet energy as the sum of each device's active training power, communication power, and idle waiting power multiplied by their respective durations, with active power calibrated from Jetson AGX Orin datasheets (60\,W at MAXN, 30\,W at 30W mode, 15\,W at 15W mode, 5\,W for low-end IoT) and idle power set to 20\% of the active level. This datasheet-based model provides an upper-bound estimate; real-device energy profiling with hardware power monitors is presented in the deployment study (Section~\ref{sec:conclusion}).


\subsection{Main Results}

% ============================================================
% Table II: Backbone 1 (CNN full-parameter)
% ============================================================
\begin{table*}[t]
\centering
\setlength{\tabcolsep}{6pt}
\renewcommand\arraystretch{1.15}
\caption{Main results with Backbone~1 (lightweight CNN, full-parameter training). Best in \best{red}, runner-up in \second{blue}. $^\dagger$Rare-Mod F1: PAMAP2 avg(Mag, HR). TTA: rounds to reach 85\% F1.}
\label{tab:main_cnn}
\resizebox{0.95\linewidth}{!}{
\begin{tabular}{l|ccc|c|c|c|c}
\Xhline{1.2pt}
\rowcolor{CadetBlue!20}
\textbf{Method} & \textbf{PAMAP2 F1 (\%)} & \textbf{MHEALTH F1 (\%)} & \textbf{Rare-Mod F1 (\%)$^\dagger$} & \textbf{Speedup} & \textbf{TTA (rds)} & \textbf{Comm (MB)} & \textbf{Energy (J)} \\
\Xhline{1.2pt}
FedAvg \venue{AISTATS'17}~\cite{McMahan2017AISTATS} & \second{92.0}\std{0.38} & 91.6\std{0.45} & 37.5\std{0.92} & 1.00$\times$ & 75 & 4.81 & 847 \\
\rowcolor{gray!10}
FedProx \venue{MLSys'20}~\cite{Li2020MLSys} & \best{92.5}\std{0.31} (\up{0.5}) & 91.7\std{0.42} (\up{0.1}) & 38.2\std{0.88} (\up{0.7}) & 1.00$\times$ & \second{65} & 4.81 & 852 \\
\hline
FedEL \venue{NeurIPS'25}~\cite{Zhang2025NeurIPS} & 81.6\std{1.05} (\down{10.4}) & 62.2\std{1.42} (\down{29.4}) & 15.3\std{1.37} (\down{22.2}) & \best{6.83$\times$} & --- & \best{3.51} & \best{198} \\
\rowcolor{gray!10}
FedICU \venue{ICML'25}~\cite{Liao2025ICML} & 87.6\std{0.62} (\down{4.4}) & 89.6\std{0.53} (\down{2.0}) & 28.4\std{1.05} (\down{9.1}) & 1.15$\times$ & 120 & \second{3.85} & 761 \\
DarkDistill \venue{KDD'25}~\cite{Qu2025KDD} & 91.3\std{0.35} (\down{0.7}) & \second{92.5}\std{0.32} (\up{0.9}) & 35.8\std{0.91} (\down{1.7}) & 1.82$\times$ & 70 & 4.81 & 523 \\
\hline
\rowcolor{gray!10}
Harmony \venue{MobiSys'23}~\cite{Ouyang2023MobiSys} & 88.2\std{0.71} (\down{3.8}) & 88.8\std{0.64} (\down{2.8}) & \second{42.6}\std{1.12} (\up{5.1}) & 1.00$\times$ & 110 & 4.81 & 839 \\
Pilot \venue{AAAI'25}~\cite{Xiong2025AAAI} & 91.8\std{0.29} (\down{0.2}) & 91.0\std{0.41} (\down{0.6}) & 34.2\std{0.86} (\down{3.3}) & 1.00$\times$ & 60 & 4.81 & 855 \\
\rowcolor{gray!10}
FedSA-LoRA \venue{ICLR'25}~\cite{Guo2025ICLR} & 92.0\std{0.33} (\up{0.0}) & 90.6\std{0.47} (\down{1.0}) & 36.8\std{0.85} (\down{0.7}) & 1.00$\times$ & 70 & 4.81 & 844 \\
HeLoRA \venue{TOIT'25}~\cite{Fan2025TOIT} & 90.4\std{0.48} (\down{1.6}) & 90.7\std{0.39} (\down{0.9}) & 33.5\std{0.98} (\down{4.0}) & 1.45$\times$ & 85 & 4.22 & 614 \\
\rowcolor{gray!10}
FedLEASE \venue{NeurIPS'25}~\cite{Wang2025NeurIPS} & 91.0\std{0.36} (\down{1.0}) & 91.2\std{0.40} (\down{0.4}) & 35.1\std{0.90} (\down{2.4}) & 1.00$\times$ & 75 & 4.81 & 851 \\
\hline
\textbf{\method{} (Ours)} & 90.1\std{0.42} (\down{1.9}) & \best{93.7}\std{0.28} (\up{2.1}) & \best{52.8}\std{1.15} (\up{15.3}) & \second{2.87$\times$} & \best{55} & 4.76 & \second{312} \\
\Xhline{1.2pt}
\end{tabular}}
\end{table*}

% ============================================================
% Table III: Backbone 2 (MOMENT + LoRA/MDLoRA)
% ============================================================
\begin{table*}[t]
\centering
\setlength{\tabcolsep}{6pt}
\renewcommand\arraystretch{1.15}
\caption{Main results with Backbone~2 (MOMENT + LoRA/MDLoRA). Best in \best{red}, runner-up in \second{blue}. $^\dagger$Rare-Mod F1: PAMAP2 avg(Mag, HR). Save relative to FedAvg-LoRA.}
\label{tab:main_lora}
\resizebox{0.98\linewidth}{!}{
\begin{tabular}{l|ccc|c|c|c|c|c}
\Xhline{1.2pt}
\rowcolor{CadetBlue!20}
\textbf{Method} & \textbf{PAMAP2 F1 (\%)} & \textbf{MHEALTH F1 (\%)} & \textbf{Rare-Mod F1 (\%)$^\dagger$} & \textbf{Speedup} & \textbf{Comm (KB)} & \textbf{Train. (\%)} & \textbf{Save (\%)} & \textbf{Energy (J)} \\
\Xhline{1.2pt}
FedAvg \venue{AISTATS'17}~\cite{McMahan2017AISTATS} & \best{78.3}\std{0.52} & 63.2\std{0.68} & 4.4\std{0.35} & 1.00$\times$ & 5457 & 0.98 & 0.0 & 1284 \\
\rowcolor{gray!10}
FedProx \venue{MLSys'20}~\cite{Li2020MLSys} & 77.8\std{0.48} (\down{0.5}) & \second{62.9}\std{0.71} (\down{0.3}) & \second{5.1}\std{0.42} (\up{0.7}) & 1.00$\times$ & 5457 & 0.98 & 0.0 & 1291 \\
\hline
FedEL \venue{NeurIPS'25}~\cite{Zhang2025NeurIPS} & 58.4\std{1.35} (\down{19.9}) & 42.1\std{1.52} (\down{21.1}) & 1.2\std{0.28} (\down{3.2}) & \second{7.68$\times$} & \second{2876} & \best{0.48} & \second{47.3} & \second{245} \\
\rowcolor{gray!10}
FedICU \venue{ICML'25}~\cite{Liao2025ICML} & 56.3\std{0.91} (\down{22.0}) & 51.6\std{0.85} (\down{11.6}) & 1.4\std{0.22} (\down{3.0}) & 1.12$\times$ & 4365 & 0.79 & 20.0 & 1158 \\
DarkDistill \venue{KDD'25}~\cite{Qu2025KDD} & 63.8\std{0.78} (\down{14.5}) & 54.5\std{0.82} (\down{8.7}) & 1.8\std{0.31} (\down{2.6}) & 1.68$\times$ & 5457 & 0.72 & 0.0 & 802 \\
\hline
\rowcolor{gray!10}
Harmony \venue{MobiSys'23}~\cite{Ouyang2023MobiSys} & 37.7\std{1.24} (\down{40.6}) & 22.3\std{1.38} (\down{40.9}) & 0.9\std{0.18} (\down{3.5}) & 1.00$\times$ & 5457 & 0.98 & 0.0 & 1276 \\
Pilot \venue{AAAI'25}~\cite{Xiong2025AAAI} & 64.2\std{0.75} (\down{14.1}) & 55.1\std{0.80} (\down{8.1}) & 1.6\std{0.27} (\down{2.8}) & 1.00$\times$ & 5821 & 1.05 & $-$6.7 & 1302 \\
\rowcolor{gray!10}
FedSA-LoRA \venue{ICLR'25}~\cite{Guo2025ICLR} & \second{78.1}\std{0.50} (\down{0.2}) & 53.3\std{0.79} (\down{9.9}) & 4.2\std{0.38} (\down{0.2}) & 1.00$\times$ & 5457 & 0.98 & 0.0 & 1280 \\
HeLoRA \venue{TOIT'25}~\cite{Fan2025TOIT} & 61.4\std{0.82} (\down{16.9}) & 52.8\std{0.84} (\down{10.4}) & 1.5\std{0.26} (\down{2.9}) & 1.35$\times$ & 4092 & \second{0.71} & 25.0 & 963 \\
\rowcolor{gray!10}
FedLEASE \venue{NeurIPS'25}~\cite{Wang2025NeurIPS} & 65.1\std{0.72} (\down{13.2}) & 56.2\std{0.76} (\down{7.0}) & 1.7\std{0.29} (\down{2.7}) & 1.00$\times$ & 5638 & 1.02 & $-$3.3 & 1295 \\
\hline
\textbf{\method{} (Ours)} & 74.9\std{0.58} (\down{3.4}) & \best{83.4}\std{0.45} (\up{20.2}) & \best{12.3}\std{0.95} (\up{7.9}) & \best{9.41$\times$} & \best{3408} & 0.61 & \best{37.5} & \best{178} \\
\Xhline{1.2pt}
\end{tabular}}
\end{table*}

% ============================================================
% Fig 5: Convergence curves, 2×2 (datasets × backbones)
% ============================================================
\begin{figure*}[t]
\centering
\subfloat[PAMAP2, B1\label{fig:conv_p_b1}]{%
    \includegraphics[width=0.24\textwidth]{figures/conv_pamap2_b1.pdf}
    }
\hfill
\subfloat[MHEALTH, B1\label{fig:conv_m_b1}]{%
    \includegraphics[width=0.24\textwidth]{figures/conv_mhealth_b1.pdf}
    }
\hfill
\subfloat[PAMAP2, B2\label{fig:conv_p_b2}]{%
    \includegraphics[width=0.24\textwidth]{figures/conv_pamap2_b2.pdf}
    }
\hfill
\subfloat[MHEALTH, B2\label{fig:conv_m_b2}]{%
    \includegraphics[width=0.24\textwidth]{figures/conv_mhealth_b2.pdf}
    }
\caption{Convergence comparison (macro-F1 vs.\ communication round) for five representative methods across two datasets and two backbones.}
\label{fig:convergence}
\end{figure*}

To answer whether \method{} achieves a favorable accuracy-speedup-energy trade-off against state-of-the-art methods, Tables~\ref{tab:main_cnn} and~\ref{tab:main_lora} compare 11 methods across two backbones and two datasets. Under Backbone~1, \method{} attains 93.7\% F1 on MHEALTH (the highest among all methods) with 2.87$\times$ wall-clock speedup and 63\% energy reduction (312\,J vs.\ 847\,J). On PAMAP2, it trades 1.9\,pp relative to FedAvg for that same 2.87$\times$ acceleration. FedEL~\cite{Zhang2025NeurIPS} is faster (6.83$\times$) and more energy-efficient (198\,J), but its F1 collapses to 81.6\% on PAMAP2 and 62.2\% on MHEALTH because its modality-unaware tensor selection assigns weak devices to train parameters for absent sensors. Under Backbone~2, FedEL's speedup advantage reverses (7.68$\times$ vs.\ \method{}'s 9.41$\times$): the CNN backbone offers many tensor-level parameter groups for FedEL to prune aggressively, whereas LoRA's compact structure limits the pruning headroom. \method{}'s modality-aligned decomposition, by contrast, maps directly onto the LoRA column-block structure and scales its elastic budget with the number of modalities rather than arbitrary tensor importance.

Backbone~2 amplifies the contrast. Most baselines that performed within 2\,pp of FedAvg under Backbone~1 (e.g., DarkDistill, FedLEASE, Pilot) drop 13--16\,pp below FedAvg under LoRA, because LoRA's compact parameter space leaves less room to absorb zero-gradient noise from missing modalities. \method{} is the only method that maintains competitive F1 on PAMAP2 (74.9\% vs.\ FedAvg 78.3\%) while achieving 9.41$\times$ speedup and 37.5\% communication savings. Note that under Backbone~1, communication savings are minimal (4.76 vs.\ 4.81\,MB) because the CNN's fusion layer accounts for a small fraction of the total parameters; the savings become pronounced under Backbone~2, where LoRA parameters dominate and per-device upload scales with $|\mathcal{M}_n|$. On MHEALTH, \method{} surpasses FedAvg by 20.2\,pp (83.4\% vs.\ 63.2\%), because ECG and IMU signals occupy different feature spaces, which intensifies cross-modal interference under FedAvg and makes cohort-wise aggregation proportionally more beneficial.

The Rare-Mod F1 column reveals that \method{} improves the average F1 of rare modalities (Mag+HR on PAMAP2, Mag+ECG on MHEALTH) by 15.3\,pp over FedAvg under Backbone~1 (52.8\% vs.\ 37.5\%) and 7.9\,pp under Backbone~2 (12.3\% vs.\ 4.4\%). Harmony~\cite{Ouyang2023MobiSys}, the runner-up on Rare-Mod F1 under Backbone~1 (42.6\%), provides no speedup. This confirms that cohort-wise aggregation is the primary driver of rare-modality gains.

To verify that \method{}'s final-round gains are not artifacts of a single checkpoint, Fig.~\ref{fig:convergence} shows the convergence trajectories across all four dataset-backbone combinations. Under Backbone~1, \method{} converges at a rate comparable to FedAvg on PAMAP2 and faster on MHEALTH, where it overtakes all baselines by round 40. FedEL converges quickly in wall-clock time but plateaus at a low F1 with persistent oscillation, reflecting the instability of modality-unaware parameter selection. Under Backbone~2, the gap between \method{} and the baselines widens: Harmony collapses to 38\%/22\% because it excludes the fusion layer from federation, and under LoRA the fusion layer contains most of the trainable parameters. \method{} is the only method that reaches above 70\% on both LoRA settings, confirming that MDLoRA's modality-aware decomposition is essential when the parameter budget is small. We note that the lower absolute F1 under Backbone~2 reflects domain mismatch between MOMENT's pretraining corpus (general time-series) and HAR sensor signals, not a limitation of \method{}. The purpose of Backbone~2 experiments is to validate that \method{}'s modality-aware mechanisms transfer to LoRA-based parameter-efficient settings, not to advocate this specific backbone for deployment.


\subsection{Ablation Study}

% ============================================================
% Table IV: Ablation — both backbones (table*)
% ============================================================
\begin{table*}[t]
\centering
\setlength{\tabcolsep}{4pt}
\renewcommand\arraystretch{1.15}
\caption{Ablation study. Arrows show delta relative to V0 (full \method{}).}
\label{tab:ablation}
\resizebox{0.95\linewidth}{!}{
\begin{tabular}{cl|ccc|ccc}
\Xhline{1.2pt}
\rowcolor{CadetBlue!20}
& & \multicolumn{3}{c|}{\textbf{Backbone~1 (CNN)}} & \multicolumn{3}{c}{\textbf{Backbone~2 (LoRA)}} \\
\rowcolor{CadetBlue!20}
& \textbf{Variant} & \textbf{PAMAP2 F1 (\%)} & \textbf{MHEALTH F1 (\%)} & \textbf{Speedup} & \textbf{PAMAP2 F1 (\%)} & \textbf{MHEALTH F1 (\%)} & \textbf{Speedup} \\
\Xhline{1.2pt}
V0 & \method{} (full) & 90.1\std{0.42} & 93.7\std{0.28} & 2.87$\times$ & 74.9\std{0.58} & 83.4\std{0.45} & 9.41$\times$ \\
\rowcolor{gray!10}
V1 & w/o elastic training & 94.0\std{0.25} (\up{3.9}) & 95.5\std{0.19} (\up{1.8}) & 1.66$\times$ & 78.5\std{0.45} (\up{3.6}) & 85.7\std{0.33} (\up{2.3}) & 1.52$\times$ \\
V2 & w/o cohort-wise agg. & 83.7\std{0.89} (\down{6.4}) & 86.5\std{0.78} (\down{7.2}) & 3.84$\times$ & 66.8\std{1.15} (\down{8.1}) & 73.8\std{1.05} (\down{9.6}) & 12.6$\times$ \\
\rowcolor{gray!10}
V3 & random elastic alloc. & 83.1\std{0.95} (\down{7.0}) & 85.5\std{0.88} (\down{8.2}) & 3.84$\times$ & 65.3\std{1.22} (\down{9.6}) & 72.1\std{1.19} (\down{11.3}) & 12.6$\times$ \\
\Xhline{1.2pt}
\end{tabular}}
\end{table*}

To understand which component drives the performance gains, Table~\ref{tab:ablation} isolates the contribution of each component across both datasets and backbones. Removing cohort-wise aggregation (V2) drops F1 by 6.4--7.2\,pp under Backbone~1 and 8.1--9.6\,pp under Backbone~2, which confirms that the compact LoRA parameter space is more sensitive to cross-modal gradient interference. The drop is larger on MHEALTH ($-$7.2/$-$9.6\,pp) than PAMAP2 ($-$6.4/$-$8.1\,pp), consistent with MHEALTH's smaller ECG cohort (3 of 10 devices) that amplifies aggregation noise. Using random instead of divergence-guided allocation (V3) causes the largest overall drop ($-$7.0 to $-$8.2\,pp on B1, $-$9.6 to $-$11.3\,pp on B2), which shows that both components are essential. V2 and V3 share the same elastic budget $k_n$ and hence the same speedup (3.84$\times$/12.6$\times$), which exceeds V0's 2.87$\times$/9.41$\times$ because V0's mandatory inclusion constraint requires each device to train all its available fusion blocks and raises the minimum workload. V2 and V3 lack this constraint, so they allow more aggressive pruning at the cost of accuracy.

Disabling elastic training (V1) raises F1 by 1.8--3.9\,pp but cuts speedup from 2.87$\times$/9.41$\times$ to 1.66$\times$/1.52$\times$, and increases per-round energy from 312\,J to 578\,J under Backbone~1. The F1 gain is smaller on MHEALTH (+1.8/+2.3\,pp) than PAMAP2 (+3.9/+3.6\,pp) because MHEALTH's higher baseline leaves less room for improvement. This trade-off is by design: elastic training exchanges a small F1 margin for substantial wall-clock and energy gains. In latency-sensitive IoT deployments, V0 is justified by 2.87$\times$ faster rounds; in accuracy-critical scenarios, V1 (cohort-wise aggregation without elastic) remains a strong standalone option.


\subsection{Sensitivity Analysis}

% ============================================================
% Table V: Sensitivity — heterogeneity + scalability, both backbones (table*)
% ============================================================
\begin{table*}[t]
\centering
\setlength{\tabcolsep}{4pt}
\renewcommand\arraystretch{1.15}
\caption{Sensitivity analysis on PAMAP2. F1 (\%) under varying heterogeneity and client count.}
\label{tab:sens_pamap2}
\resizebox{0.95\linewidth}{!}{
\begin{tabular}{ll|ccccc|ccccc}
\Xhline{1.2pt}
\rowcolor{CadetBlue!20}
& & \multicolumn{5}{c|}{\textbf{Backbone~1 (CNN)}} & \multicolumn{5}{c}{\textbf{Backbone~2 (LoRA)}} \\
\rowcolor{CadetBlue!20}
\textbf{Factor} & \textbf{Setting} & \textbf{FedAvg} & \textbf{FedEL} & \textbf{Harmony} & \textbf{DarkDist.} & \textbf{\method{}} & \textbf{FedAvg} & \textbf{FedEL} & \textbf{Harmony} & \textbf{DarkDist.} & \textbf{\method{}} \\
\Xhline{1.2pt}
Hetero. & Mild (10$\times$) & 92.1\std{0.37} & 82.4\std{1.02} & 88.5\std{0.68} & 91.5\std{0.41} & \cellcolor{green!8}90.4\std{0.39} & 78.8\std{0.48} & 60.2\std{1.22} & 38.9\std{1.15} & 64.5\std{0.79} & \cellcolor{green!8}75.6\std{0.54} \\
\rowcolor{gray!10}
& Moderate (55$\times$) & 92.0\std{0.38} & 81.6\std{1.05} & 88.2\std{0.71} & 91.3\std{0.35} & \cellcolor{green!8}90.1\std{0.42} & 78.3\std{0.52} & 58.4\std{1.35} & 37.7\std{1.24} & 63.8\std{0.78} & \cellcolor{green!8}74.9\std{0.58} \\
& Extreme (100$\times$) & 91.6\std{0.43} & 80.9\std{1.18} & 87.8\std{0.82} & 90.7\std{0.39} & \cellcolor{green!8}88.5\std{0.51} & 77.9\std{0.59} & 57.8\std{1.42} & 36.2\std{1.35} & 62.4\std{0.91} & \cellcolor{green!8}73.6\std{0.62} \\
\hline
\rowcolor{gray!10}
Scale & $N{=}8$ & 92.0\std{0.38} & 81.6\std{1.05} & 88.2\std{0.71} & 91.3\std{0.35} & \cellcolor{green!8}90.1\std{0.42} & 78.3\std{0.52} & 58.4\std{1.35} & 37.7\std{1.24} & 63.8\std{0.78} & \cellcolor{green!8}74.9\std{0.58} \\
& $N{=}20$ & 91.4\std{0.40} & 80.2\std{1.15} & 87.5\std{0.79} & 90.6\std{0.38} & \cellcolor{green!8}89.6\std{0.45} & 77.6\std{0.55} & 57.1\std{1.38} & 35.8\std{1.28} & 62.1\std{0.85} & \cellcolor{green!8}74.2\std{0.61} \\
\rowcolor{gray!10}
& $N{=}50$ & 90.5\std{0.49} & 78.8\std{1.28} & 86.1\std{0.88} & 89.4\std{0.46} & \cellcolor{green!8}88.7\std{0.53} & 76.8\std{0.64} & 55.6\std{1.52} & 33.5\std{1.41} & 60.2\std{0.98} & \cellcolor{green!8}73.4\std{0.66} \\
& $N{=}100$ & 89.8\std{0.54} & 77.1\std{1.35} & 84.8\std{0.95} & 88.5\std{0.52} & \cellcolor{green!8}88.2\std{0.57} & 76.1\std{0.70} & 54.2\std{1.58} & 31.8\std{1.48} & 58.5\std{1.05} & \cellcolor{green!8}72.8\std{0.72} \\
\Xhline{1.2pt}
\end{tabular}}
\end{table*}

% ============================================================
% Table VI: Sensitivity on MHEALTH
% ============================================================
\begin{table*}[t]
\centering
\setlength{\tabcolsep}{4pt}
\renewcommand\arraystretch{1.15}
\caption{Sensitivity analysis on MHEALTH. F1 (\%) under varying heterogeneity and client count.}
\label{tab:sens_mhealth}
\resizebox{0.95\linewidth}{!}{
\begin{tabular}{ll|ccccc|ccccc}
\Xhline{1.2pt}
\rowcolor{CadetBlue!20}
& & \multicolumn{5}{c|}{\textbf{Backbone~1 (CNN)}} & \multicolumn{5}{c}{\textbf{Backbone~2 (LoRA)}} \\
\rowcolor{CadetBlue!20}
\textbf{Factor} & \textbf{Setting} & \textbf{FedAvg} & \textbf{FedEL} & \textbf{Harmony} & \textbf{DarkDist.} & \textbf{\method{}} & \textbf{FedAvg} & \textbf{FedEL} & \textbf{Harmony} & \textbf{DarkDist.} & \textbf{\method{}} \\
\Xhline{1.2pt}
Hetero. & Mild (10$\times$) & 91.8\std{0.42} & 63.5\std{1.32} & 89.1\std{0.65} & 92.8\std{0.33} & \cellcolor{green!8}94.0\std{0.31} & 63.8\std{0.62} & 43.5\std{1.48} & 23.8\std{1.28} & 55.7\std{0.85} & \cellcolor{green!8}83.8\std{0.44} \\
\rowcolor{gray!10}
& Moderate (55$\times$) & 91.6\std{0.45} & 62.2\std{1.42} & 88.8\std{0.64} & 92.5\std{0.32} & \cellcolor{green!8}93.7\std{0.28} & 63.2\std{0.68} & 42.1\std{1.52} & 22.3\std{1.38} & 54.5\std{0.82} & \cellcolor{green!8}83.4\std{0.45} \\
& Extreme (100$\times$) & 91.3\std{0.47} & 61.5\std{1.55} & 88.1\std{0.78} & 91.6\std{0.38} & \cellcolor{green!8}92.1\std{0.41} & 62.5\std{0.75} & 41.2\std{1.58} & 21.5\std{1.45} & 53.2\std{0.93} & \cellcolor{green!8}81.5\std{0.54} \\
\hline
\rowcolor{gray!10}
Scale & $N{=}10$ & 91.6\std{0.45} & 62.2\std{1.42} & 88.8\std{0.64} & 92.5\std{0.32} & \cellcolor{green!8}93.7\std{0.28} & 63.2\std{0.68} & 42.1\std{1.52} & 22.3\std{1.38} & 54.5\std{0.82} & \cellcolor{green!8}83.4\std{0.45} \\
& $N{=}20$ & 91.0\std{0.48} & 60.8\std{1.48} & 87.9\std{0.75} & 91.8\std{0.36} & \cellcolor{green!8}93.1\std{0.34} & 62.4\std{0.71} & 40.5\std{1.62} & 20.8\std{1.42} & 52.8\std{0.89} & \cellcolor{green!8}82.1\std{0.52} \\
\rowcolor{gray!10}
& $N{=}50$ & 90.1\std{0.53} & 57.3\std{1.65} & 86.5\std{0.85} & 90.4\std{0.44} & \cellcolor{green!8}92.0\std{0.38} & 61.2\std{0.78} & 38.2\std{1.68} & 18.9\std{1.55} & 50.6\std{0.97} & \cellcolor{green!8}80.5\std{0.61} \\
& $N{=}100$ & 89.4\std{0.60} & 54.6\std{1.75} & 85.2\std{0.92} & 89.1\std{0.51} & \cellcolor{green!8}91.2\std{0.48} & 60.3\std{0.85} & 36.1\std{1.78} & 17.2\std{1.62} & 48.3\std{1.05} & \cellcolor{green!8}79.2\std{0.68} \\
\Xhline{1.2pt}
\end{tabular}}
\end{table*}

Real-world IoT deployments vary in device heterogeneity and fleet size. To assess whether \method{} remains effective under these variations, Tables~\ref{tab:sens_pamap2} and~\ref{tab:sens_mhealth} examine robustness on both datasets across five representative methods. As the compute gap widens from 10$\times$ to 100$\times$, FedAvg F1 remains nearly constant (it always waits for the slowest device to finish the full model), while FedEL drops steadily (82.4$\to$80.9\% on PAMAP2 B1, 63.5$\to$61.5\% on MHEALTH B1). Harmony degrades under Backbone~2 because its fusion-layer exclusion becomes more costly as heterogeneity grows. \method{} degrades by only 1.9\,pp on PAMAP2 (90.4$\to$88.5\%) and 1.9\,pp on MHEALTH (94.0$\to$92.1\%) under Backbone~1, maintaining the best accuracy-robustness trade-off.

Increasing $N$ from 8 to 100 reduces all methods' F1 as data becomes more fragmented. FedEL degrades most sharply ($-$4.5\,pp on PAMAP2, $-$7.6\,pp on MHEALTH under Backbone~1) because modality-unaware elastic selection makes more errors with more heterogeneous devices. Harmony under Backbone~2 collapses from 22.3\% to 17.2\% on MHEALTH, confirming its inability to scale without federating the fusion layer. \method{} drops only 1.9\,pp on PAMAP2 and 2.5\,pp on MHEALTH under Backbone~1, and its advantage over FedAvg on MHEALTH persists at all fleet sizes (83.4$\to$79.2\% vs.\ 63.2$\to$60.3\% under Backbone~2).


\subsection{In-Depth Analysis}

% ============================================================
% Fig 6: Per-modality F1 breakdown, 2×2
% ============================================================
\begin{figure*}[t]
\centering
\subfloat[PAMAP2, B1\label{fig:pmod_p_b1}]{%
    \includegraphics[width=0.24\textwidth]{figures/permod_pamap2_b1.pdf}
    }
\hfill
\subfloat[MHEALTH, B1\label{fig:pmod_m_b1}]{%
    \includegraphics[width=0.24\textwidth]{figures/permod_mhealth_b1.pdf}
    }
\hfill
\subfloat[PAMAP2, B2\label{fig:pmod_p_b2}]{%
    \includegraphics[width=0.24\textwidth]{figures/permod_pamap2_b2.pdf}
    }
\hfill
\subfloat[MHEALTH, B2\label{fig:pmod_m_b2}]{%
    \includegraphics[width=0.24\textwidth]{figures/permod_mhealth_b2.pdf}
    }
\caption{Per-modality F1 breakdown. \method{} yields the largest gains on rare modalities (Mag, HR, ECG), consistent with the theoretical prediction that cohort-wise aggregation benefits smaller cohorts more.}
\label{fig:permod_f1}
\end{figure*}

The aggregate Rare-Mod F1 in Tables~\ref{tab:main_cnn}--\ref{tab:main_lora} shows that \method{} benefits rare modalities, but does not reveal whether this comes at the expense of common modalities or how individual modalities respond. Fig.~\ref{fig:permod_f1} answers this by breaking down F1 by modality across all four dataset-backbone combinations. Across all settings, Acc F1 varies by less than 3\,pp between methods (all devices contribute Acc gradients), confirming that cohort-wise aggregation does not harm shared modalities. In contrast, Mag, HR, and ECG F1 show large gaps: under Backbone~1 on PAMAP2, \method{} improves Mag F1 by 15.4\,pp and HR F1 by 15.2\,pp over FedAvg, while Acc improves by only 1.7\,pp. Under Backbone~2 on MHEALTH, Mag F1 jumps from 1.7\% (FedAvg) to 16.9\% (\method{}), and ECG from 1.6\% to 7.8\%. Harmony~\cite{Ouyang2023MobiSys} also improves rare modalities under Backbone~1 (it separates encoder training by modality), but collapses under Backbone~2 because it excludes the fusion layer from federation. The disproportionate gain on rare modalities is consistent with Theorem~\ref{thm:convergence}: the cohort residual $(\sigma^2/E + \zeta_m^2)/|\tilde{\mathcal{C}}_m|$ decreases faster for small cohorts when $|\tilde{\mathcal{C}}_m|$ is enlarged through divergence-guided allocation.


==> section/6_conclusion.tex <==
\section{Conclusion}\label{sec:con}

